Verifying linear temporal specifications of constant-rate multi-mode systems

Constant-rate multi-mode systems (MMS) are hybrid systems with finitely many modes and real-valued variables that evolve over continuous time according to mode-specific constant rates. We introduce a variant of linear temporal logic (LTL) for MMS, and we investigate the complexity of the model-checking problem for syntactic fragments of LTL. We obtain a complexity landscape where each fragment is either P-complete, NP-complete or undecidable. These results generalize and unify several results on MMS and continuous counter systems.

==> sec-undecidable.tex <==

\newcommand{\gvfrag}{\fragment{\G, \lor}}
\newcommand{\ufrag}{\fragment{\U}}

This section is dedicated to proving undecidability of the fragments
\gvfrag\ and \ufrag. Both reductions are from problems dealing with
reset Petri nets, namely termination for \gvfrag\ and reachability for
\ufrag. In both cases, the MMS defined for a given reset Petri net are
almost identical. The core of both reductions is a construction that,
given a reset Petri net, defines an MMS such that executions of a
specific shape in the MMS correspond to runs in the reset Petri
net. It then remains to define formulas of \gvfrag\ and \ufrag\ that
restrict executions to the specific shape, and to encode either
termination or reachability.

Let us first present the construction of the MMS. Let $\pn = (P, T, F,
R)$ be a reset Petri net. Let $\msrc, \mtgt$ be respectively the
source and target configurations. We will define an $(|P| + |T| +
4)$-dimensional MMS $\M$.

\paragraph*{Dimensions.}

Each of the first $|P|$ dimensions is associated to some $p \in P$,
and each of the next $|T|$ ones is associated to some $t \in T$. We
refer to these $|P|$ and $|T|$ dimensions as $\vec{p}$ and
$\vec{t}$. The last four dimensions are $u, \overline{u}$, $s$ and
$r$.

Intuitively, dimension $u$ and $\overline{u}$ count how many
transitions have been fired, and will move in lockstep. Counter $s$
counts, while firing a transition, by how much the transition was
applied so far. Roughly speaking, we increase counter $s$ as a
transition is fired. To ensure the transition is fired fully, we
require that $s = 1$ holds after firing the transition. When this is
the case, we allow increasing $\overline{u}$ until $u = \overline{u}$,
and a new transition can be fired. Dimension $s$ serves to enable this
careful manipulation of $u$ in relation to $\overline{u}$.

Dimension $r$ is used to facilitate reset transitions. It is increased
to decrement places that are reset by a transition after we have
realized its effect, and is restricted to be equal to zero everywhere
else, thus disabling the modes used for decrementing. We use $\vec{p}$
to store the current configuration, and we keep $\vec{t} \in [0, 1]^n$
with at most one nonzero dimension at any point in time.

\paragraph*{Zones.}

\newcommand{\Zi}[1]{Z_{t,#1}}
\newcommand{\Ti}[1]{T_{t,#1}}
\newcommand{\Ri}{R_t}

Let us define $1 + 6 \abs{T}$ zones. First, zone $B$ is defined by
these constraints:
\[
\begin{array}{lp{2pt}llllll}
  \toprule
  && \vec{p} & \vec{t} & u & s & r \\
  \midrule
  %
  B && \geq \vec{0} & = \vec{0} & = \overline{u} & = 0 & = 0 \\
  %
  \bottomrule
\end{array}
\]

Next, for each $t \in T$, we define zones $\Zi{1}$, $\Ti{1}$,
$\Zi{2}$, $\Ti{2}$, $\Ri$ and $\Ti{3}$. Each of these zones requires
$\vec{p} \geq 0$ and $\vec{t}(t') = 0$ for all $t' \neq t$. They also
have these additional constraints:
\[
\begin{array}{lp{2pt}llllll}
  \toprule
  && t & u & s & r \\
  \midrule
  %
  \Ti{1} && \in (0, 1) & = \overline{u} & \in (0, 1) & = 0 \\
  \Zi{1} && = 1 & = \overline{u} & = 1 & = 0 \\
  \Ti{2} && \in (0, 1) & \in (\overline{u}, \overline{u} + 1) & = 1 & = 0 \\
  \Zi{2} && = 0 & = \overline{u} + 1 & = 1 & = 0 \\
  \Ri    && \geq 0 & = \overline{u} + 1 & = 1 & \geq 0 \\
  \Ti{3} && = 0  & \in (\overline{u}, \overline{u} + 1) & \in (0, 1) & = 0 \\
  %
  \bottomrule
\end{array}
\]
Zone $\Ti{3}$ further requires that $p = 0$ for all $(p, t) \in R$.


\newcommand{\mi}[1]{\vec{a}_{t,#1}}
\newcommand{\mj}[1]{\vec{a}_{t',#1}}
\newcommand{\ei}[1]{\vec{b}_{t,#1}}
\newcommand{\ej}[1]{\vec{b}_{t',#1}}
\newcommand{\ef}{\vec{c}_{t}}
\newcommand{\efj}{\vec{c}_{t'}}

\paragraph*{Modes.}

We have three modes $\mi{1}, \mi{2}, \mi{3}$ for each transition $t$,
that are almost identical across transitions and serve to realize
adding $\effect{t}$ to $\vec{p}$. We further have $\abs{\{p : (p, t)
  \in R\}}$ modes that serve to decrement places that are reset by
$t$.\michael{I changed $\ei{p}(t)$ from $-1$ to $1$. OK?}

\[
\begin{array}{lp{2pt}ccccc}
  \toprule
  j        && \mi{1}(j)  & \mi{2}(j)  & \ei{p}(j)  & \ef(j)     & \mi{3}(j) \\
  \midrule
  \vec{p}  && \effect{t} &  \vec{0}   & -\vec{e}_p & \vec{0}    & \vec{0}   \\
  \vec{t}  && \vec{e}_t  & -\vec{e}_t & \vec{e}_t  & -\vec{e}_t & \vec{0}   \\
  u            && 0      & 1          & 0          & 0          & 0         \\
  \overline{u} && 0      & 0          & 0          & 0          & 1         \\
  s            && 1      & 0          & 0          & 0          & -1        \\
  r            && 0      & 0          & 1          & -1         & 0         \\
  \bottomrule
\end{array}
\]

\paragraph*{Executions.}

We are ready to prove that certain executions of $\M$ correspond to
runs in $\pn$.\philip{need to define "maintaining reach", i.e.  $p_1$
  reaches $p_2$ while staying in zone $\Ti{2}$.  I recall Alex also
  used this.}\philip{maintain-reach without a target means can
  maintain, but we don't care about the target since the run is
  infinite and there thus is not really a target}

\begin{lemma}\label{lem:infrun}
  Let $\pi$ be an infinite schedule, and let $\vec{x} \in B$. If
  $\vec{x} \mreach{\pi}{\AP}$, then there exists $\beta \in \Rnon$
  such that $\induced{\pi}{\vec{x}}(\beta) \in B$.
\end{lemma}

\begin{lemma}\label{lem:btob}
  Let $\vec{x}, \vec{x}' \in B$ be such that $\vec{x} \neq
  \vec{x}'$. Let $\pi$ be a schedule such that $\vec{x}
  \mreach{\pi}{\AP} \vec{x}'$ has no intermediate point in $B$. There
  exists $t \in T$ such that $\pi = (1, \mi{1}) (1,\mi{2}) \pi_R
  (1,\mi{3})$, where $\pi_R$ contains only modes of the form $\ei{p}$
  and $\ef$. Further, $\vec{x}(\vec{p}) \trans{t} \vec{x}'(\vec{p})$
  in $\pn$, and $\vec{x}'(u) = \vec{x}'(\overline{u}) = \vec{x}(u) + 1
  = \vec{x}(\overline{u}) + 1$.
\end{lemma}

\begin{proof}
  Since $\vec{x} \neq \vec{x}'$, it must be the case that $\pi$ is
  nonempty.

  The first mode used by $\pi$ must be of the form $\mi{1}$. Indeed,
  for every $t' \in T$ and $(p, t') \in R$, each of these modes leads
  outside of $\AP$ because of their non-negative constraints:
  \begin{alignat*}{4}
    \mj{2}:
    &\text{ due to } & \mj{2}(t') &= -1 && \text{ and } & \vec{x}(t') = 0; \\
    %
    \mj{3}:
    &\text{ due to } & \mj{3}(s) &= -1 && \text{ and } & \vec{x}(s) = 0; \\
    %
    \ej{p}:
    &\text{ due to } & \ej{p}(t') &= -1 && \text{ and } & \vec{x}(t') = 0; \\
    %
    \efj:
    &\text{ due to } & \ef(r) &= -1 && \text{ and } & \vec{x}(r) = 0.
  \end{alignat*}

  ...\michael{Unfinished proof.}
\end{proof}

\begin{proposition}\label{prop:simulation}
  Let $\vec{m}, \vec{m}' \in \N^P$ and $b \in \N$. It is the case that
  $\vec{m} \trans{} \vec{m}'$ in $\pn$ iff there exist $\vec{x} \in B,
  \vec{x}_1 \in \Zi{1}$, $\vec{x}_2, \vec{x}_3 \in \Zi{2}$, $\vec{x}'
  \in B$, $t \in T$ and schedules $\pi_1, \pi_2, \pi_R, \pi_3$ that
  satisfy:
  \begin{enumerate}
  \item $\vec{x}(\vec{p}) = \vec{m}$, $\vec{x}(u) =
    \vec{x}(\overline{u}) = b$;

  \item $\vec{x}'(\vec{p}) = \vec{m}'$, $\vec{x}'(u) =
    \vec{x}'(\overline{u}) = b + 1$,

  \item $\vec{x} \mreach{\pi_1}{\Ti{1}} \vec{x}_1
    \mreach{\pi_2}{\Ti{2}} \vec{x}_2 \mreach{\pi_R}{\Ri} \vec{x}_3
    \mreach{\pi_3}{\Ti{3}} \vec{x}'$.
  \end{enumerate}
\end{proposition}

\begin{proof}
  $\Leftarrow$) Let $\pi \defeq \pi_1 \pi_2 \pi_R \pi_3$. By
  assumption, $\vec{x} \mreach{\pi}{\AP \setminus \{B\}}
  \vec{x}'$.\michael{$\setminus \{B\}$ does not mean outside of $B$.} 
  Since $B$ is disjoint from the other zones from $\AP$, it follows
  that $\vec{x} \mreach{\pi}{\AP} \vec{x}'$ has no intermediate point
  in $B$.

  Since $\vec{x} \neq \vec{x}'$, \Cref{lem:btob} yields some $t \in T$
  such that $\vec{m} = \vec{x}(\vec{p}) \trans{t} \vec{x}'(\vec{p}) =
  \vec{m}'$ in $\pn$.

  $\Rightarrow$) We have $\vec{m} \trans{t} \vec{m}'$ in $\pn$ for
  some $t \in T$. Thus,
  \[
  \vec{m}'(p) =
  \begin{cases}
    0                          & \text{if } (p, t) \in R, \\
    \vec{m}(p) + \effect{t}(p) & \text{otherwise}.
  \end{cases}
  \]

  Let us define $\vec{x}$, $\vec{x}_1$, $\vec{x}_2$, $\vec{x}_3$ and
  $\vec{x}'$:
  \[
  \begin{array}{lp{2pt}llllll}
    \toprule
    && \vec{x} & \vec{x}_1 & \vec{x}_2 & \vec{x}_3 & \vec{x}' \\
    \midrule
    %
    \vec{p}      && \vec{m}  & \vec{m} + \effect{t}
                  & \vec{m} + \effect{t} & \vec{m}' & \vec{m}' \\
    
    \vec{t}      && \vec{0} & \vec{e}_t & \vec{0}  & \vec{0}  & \vec{0} \\
    u            && 0 & 0 & 1 & 1 & 1 \\
    \overline{u} && 0 & 0 & 0 & 0 & 1 \\
    s            && 0 & 1 & 1 & 1 & 0 \\
    r            && 0 & 0 & 0 & 0 & 0 \\
    %
    \bottomrule
  \end{array}
  \]

  Let $\pi_1 \defeq (1, \mi{1})$, $\pi_2 \defeq (1, \mi{2})$, $\pi_3
  \defeq (1, \mi{3})$ and
  \[
  \pi_R \defeq
  \prod_{(p, t) \in R}
  (\vec{m}(p) + \effect{t}(p), \ei{p})\,
  (\vec{m}(p) + \effect{t}(p), \ef).
  \]

  We have $\vec{x} \in B$, $\vec{x}_1 \in \Zi{1}$, $\vec{x}_2,
  \vec{x}_3 \in \Zi{2}$, $\vec{x}' \in B$, and
  \[
  \vec{x}
  \mreach{\pi_1}{\Ti{1}} \vec{x}_1
  \mreach{\pi_2}{\Ti{2}} \vec{x}_2
  \mreach{\pi_R}{\Ri}    \vec{x}_3
  \mreach{\pi_3}{\Ti{3}} \vec{x}'.\qedhere
  \]
\end{proof}

\begin{lemma}\label{lem:plusone}
  Let $b \in \N$, $\vec{x} \in B$, $\vec{x}_1 \in \Zi{1}$, $\vec{x}_2,
  \vec{x}_3 \in \Zi{2}$, $\vec{x}' \in B$ and $\pi_1, \pi_2, \pi_R,
  \pi_3$ be such that $\vec{x}(u) = \vec{x}(\overline{u}) = b$ and
  \[
  \vec{x}   \mreach{\pi_1}{\Ti{1}}
  \vec{x}_1 \mreach{\pi_2}{\Ti{2}}
  \vec{x}_2 \mreach{\pi_R}{\Ri}
  \vec{x}_3 \mreach{\pi_3}{\Ti{3}}
  \vec{x}'.
  \]
  It is the case that $\vec{x}'(u) = \vec{x}'(\overline{u}) = b +
  1$.\philip{I hope this is able to be rolled into the above
    proposition, but I'm unsure how.}
\end{lemma}

\begin{theorem}
  The fragment \fragment{\G, \lor} is undecidable.
\end{theorem}

\begin{proof}
  We give a reduction from the non-termination problem for reset Petri
  nets, which is known to be undecidable~\michael{It is
  decidable!}. Let $\pn = (P, T, F, R)$ be a reset Petri net, and let
  $\msrc$ be the initial marking. We wish to determine whether
  $m \trans{\rho}$ holds for some infinite run $\rho$.\philip{is it
  true that in any (reset) pn, one can avoid having transitions that
  consume and produce in the same place? it seems possible by
  transforming to a VASS, splitting transitions into pre and post,
  then converting back. would be nice to have a reference, in case
  this is true}

  Let $\M$ and $\AP$ be the MMS and set of zones obtained from the
  aforementioned construction. For each $t \in T$, let $\varphi_t \defeq
  \Ti{1} \lor \Zi{1} \lor \Ti{2} \lor \Zi{2} \lor \Ri \vee
  \Ti{3}$. Let
  \begin{align*}
    \varphi \defeq \G (B \lor \bigvee_{t \in T} \varphi_t).
  \end{align*}
  Let $\vec{x}_0 \in B$ be such that $\vec{x}_0(\vec{p}) \defeq \msrc$
  and $\vec{x}_0(u) = \vec{x}_0(\overline{u}) \defeq 0$. We show that
  there exists an infinite run $\rho$ such that $\msrc \trans{\rho}$
  in $\pn$ iff $\vec{x}_0 \models_M \varphi$.

  $\Rightarrow)$ By assumption, there exist $t_1, t_2, \ldots \in T$
  and $\vec{m}_0, \allowbreak \vec{m}_1, \allowbreak \ldots \in \N^P$
  such that $\msrc = \vec{m}_0 \trans{t_1} \vec{m}_1 \trans{t_2}
  \cdots$.

  For every $i \in \N_{\geq 1}$, let $\vec{x}_i \in B$ be such that
  $\vec{x}_i(\vec{p}) \defeq \vec{m}_i$ and $\vec{x}_i(u) =
  \vec{x}_i(\overline{u}) \defeq i$. By repeatedly invoking
  \Cref{prop:simulation}, we obtain schedules $\pi_0, \pi_1,
  \ldots$ such that
  \[
  \vec{x}_0
  \mreach{\pi_0}{\AP} \vec{x}_1
  \mreach{\pi_1}{\AP} \vec{x}_2
  \mreach{\pi_2}{\AP} \cdots.
  \]

  Let $\pi \defeq \pi_0 \pi_1 \cdots$. Since
  $\induced{\pi}{\vec{x}_0}$ is infinite, and each point of
  $\induced{\pi}{\vec{x}_0}$ lies in a zone of $\AP$, we have
  $\vec{x}_0 \models_\M \varphi$.
   
  $\Leftarrow)$ Since $\vec{x}_0 \models_\M \varphi$, there exists an
  infinite schedule $\pi$ such that $\induced{\pi}{\vec{x}_0} \models
  \varphi$. By definition of $\varphi$, we have $\vec{x}_0
  \mreach{\pi}{\AP}$.

  By repeatedly applying \Cref{lem:infrun}, we obtain $\beta_1 <
  \beta_2 < \cdots$ such that $\vec{x}_i \defeq
  \induced{\pi}{\vec{x}_0}(\beta_i) \in B$.

  Let $\pi \defeq \pi_1 \pi_2 \cdots$ so that $\vec{x}_i
  \mreach{\pi_{i+1}}{} \vec{x}_{i+1}$ for every $i \in \N$. Since
  $\vec{x}_0 \mreach{\pi_1}{\AP} \vec{x}_1 \mreach{\pi_2}{\AP} \dots$,
  \Cref{lem:btob} yields $\msrc = \vec{x}_0(\vec{p}) \trans{t_1}
  \vec{x}_1(\vec{p}) \trans{t_2} \cdots$ for some $t_1, t_2, \ldots
  \in T$. We are done since $\msrc \trans{\rho}$ with $\rho \defeq t_1
  t_2 \cdots$.
\end{proof}

\begin{theorem}
  The fragment \fragment{\U} is undecidable.\michael{I think we could
  have a formula of the form $(X_1 \lor X_2 \lor \cdots \lor X_n) \U
  Y$ and say that it is equivalent to some formula
  from \fragment{\U}.}
\end{theorem}

\begin{proof}
  We give a reduction from the reachability problem for reset Petri
  nets, which is known to be undecidable~\cite{AK76}. Given a reset
  Petri net $\pn = (P, T, F, R)$ and markings $\msrc, \mtgt \in \N^P$,
  we wish to determine whether $\msrc \trans{\rho} \mtgt$ in $\pn$.
  Let $\M$ and $\AP$ be the MMS and set of zones obtained from the
  aforementioned construction.

  We introduce an additional zone $F$ to allow us to detect whether
  $\mtgt$ has been reached:
  \[
  \begin{array}{lp{2pt}llllll}
    \toprule
    && \vec{p} & \vec{t} & u & s & r \\
    \midrule
    %
    F && = \mtgt & = \vec{0} & = \overline{u} & = 0 & = 0 \\
    %
    \bottomrule
  \end{array}
  \]

  We will define a formula $\varphi$ over $\AP' \defeq \AP \cup \{F\}$
  that is satisfied iff $\msrc \trans{*} \mtgt$ in $\pn$. For every $t
  \in T$, let
  \begin{multline*}
    \varphi_t \defeq
    B \U (\Ti{1} \U (\Zi{1} \U (\Ti{2} \U (\Zi{2} \U {} \\
    (\Ri \U (\Ti{3} \U B)))))).
  \end{multline*}
  Let $\varphi' \defeq \varphi_{t_1} \U (\varphi_{t_2} \U \dots \U
  (\varphi_{t_{n-1}} \U \phi_{t_n})\dots))$, where $T = \{t_1, \ldots,
  t_n\}$. Let $\varphi \defeq \varphi' \U F$.\michael{Double-check
    formulas.}

  It remains to prove that $\vec{x}_0 \models_\M \varphi$ iff $\msrc
  \trans{*} \mtgt$ in $\pn$.\michael{$\vec{x}_0$ undefined.}

  $\Rightarrow)$ By assumption, there exists a schedule $\pi$ such
  that $\induced{\vec{x}_0}{\pi} \models \varphi$. Since $\varphi =
  \varphi' \U F$, this means that $\vec{x}_0 \trans{\pi} \vec{x}'$ for
  some $\vec{x}' \in F$. If $\vec{x}_0 = \vec{x}'$, then we are done,
  as $\vec{x}_0(\vec{p}) = \msrc$, $\vec{x}'(\vec{p}) = \mtgt$, and
  hence $\msrc = \mtgt$.

  So, assume that $\vec{x}_0 \neq \vec{x}'$ and hence that $\pi$ is
  nonempty. Let $\sigma \defeq \induced{\vec{x}_0}{\pi}$. By
  definition of $\varphi$, there exists $\beta \in \Rnon$ such that
  \[
  \FromTo{\sigma}{\beta}{} \models F
  \land
  (\forall \alpha \in [0, \beta) : \FromTo{\sigma}{\alpha}{} \models
    \varphi').
  \]
  By definition of $\varphi'$, this implies that $\vec{x}_0
  \mreach{\pi}{\AP'} \vec{x}'$, \ie\ $\sigma$ stays within $\AP'$.

  Let us split $\pi$ into the parts that start and end in $B$, with no
  intermediate points in $B$. More formally, let $j_1 < j_2 < \cdots <
  j_k$ be such that for all $\ell \in [1..k]$:\michael{$\setminus
    \{B\}$ does not mean outside of $B$.}
  \[
  \vec{x}_0 \mreach{\FromTo{\pi}{}{j_\ell}}{\AP' \setminus \{B\}} \vec{x}_\ell
  \text{ with }
  \vec{x}_\ell \in B.
  \]

  As $\vec{x}' \in B$, we have $k \geq 1$ \michael{Why so? Maybe we
    never leave $B$.} and $\vec{x}_k = \vec{x}'$. Note that
  \[
  \vec{x}_0 \mreach{\FromTo{\pi}{}{j_1}}{\AP'}
  \vec{x}_1 \mreach{\FromTo{\pi}{j_1}{j_2}}{\AP'}
  \cdots
  \vec{x}_{k-1} \mreach{\FromTo{\pi}{j_{k-1}}{j_k}}{\AP'} \vec{x}',
  \]
  with no intermediate points from $B$.

  By applying \Cref{lem:btob} to each (sub)execution, we obtain
  $\vec{x}_0(\vec{p}) \trans{} \vec{x}_1(\vec{p}) \trans{} \cdots
  \vec{x}_k(\vec{p})$ in $\pn$, and thus $\msrc \trans{*} \mtgt$.

  $\Leftarrow)$ Since $\msrc \trans{*} \mtgt$, there exist $t_1, t_2,
  \ldots, t_k \in T$ and $\vec{m}_0, \vec{m}_1, \ldots, \vec{m}_k \in
  \N^P$ such that
  \[
  \msrc = \vec{m}_0 \trans{t_1} \vec{m}_1 \trans{t_2} \cdots
  \trans{t_k} \vec{m}_k = \msrc.
  \]  
  By applying \Cref{prop:simulation,lem:plusone}, we obtain
  \[
  \vec{x}_{1, 0} \mreach{\pi_{1, 1}}{T_{t_1, 1}}
  \vec{x}_{1, 1} \mreach{\pi_{1, 2}}{T_{t_1, 2}}
  \vec{x}_{1, 2} \mreach{\pi_{1, R}}{\Ri}
  \vec{x}_{1, 3} \mreach{\pi_{1, 3}}{T_{t_1, 3}}
  \vec{x}_{1, 4},
  \]
  for some $\vec{x}_{1, 0} \in B$, $\vec{x}_{1, 1} \in Z_{t_1, 1}$,
  $\vec{x}_{1, 2}, \vec{x}_{1, 3} \in Z_{t_1, 2}$ and $\vec{x}_{1, 4}
  \in B$ with $\vec{x}_{1, 0}(\vec{p}) = \vec{m}_0$ and $\vec{x}_{1,
    4}(\vec{p}) = \vec{m}_1$.

  We can further choose to fix $\vec{x}_{1, 0}(u) = \vec{x}_{1,
    0}(\overline{u}) = 0$ and $\vec{x}_{1, 4}(u) = \vec{x}_{1,
    4}(\overline{u}) = 1$. Observe that $\induced{\pi_{1, 1} \pi_{1,
    2} \pi_{1, R} \pi_{1, 3}}{\vec{x}_{1, 0}}$ satisfies
    $\varphi_{t_1}$.
  
  By a similar argument, we get schedules $\pi_{2, 1} \pi_{2,
  2} \pi_{2, R} \pi_{2, 3}$ such that $\induced{\pi_{2, 1} \pi_{2,
  2} \pi_{2, R} \pi_{2, 3}}{\vec{x}_{1,4}}$ satisfies $\varphi_{t_2}$,
  and so on. For ease of notation, let $\sigma_i \defeq \pi_{i,
  1} \pi_{i, 2} \pi_{i, 3} \pi_{i, 4}$.

  By the choice of $\sigma_1, \dots, \sigma_n$ and
  by \Cref{prop:simulation}, it must hold that $\vec{x}_{1,
  0} \trans{\sigma_1 \dots \sigma_n} \vec{x}_{n, 4}$ with $\vec{x}_{n,
  4} \in B$ and $\vec{x}_{n, 4}(\vec{p}) = \mtgt$. By comparing the
  constraints of $B$ and $F$, it is clear that $\vec{x}_{n, 4} \in F$.
  Thus,
  $\induced{\sigma_1 \cdots \sigma_n}{\vec{x}_0} \models \varphi' \U F
  = \varphi$.
\end{proof}

